FOFO: A Benchmark to Evaluate LLMs' Format-Following Capability

This paper presents FoFo, a pioneering benchmark for evaluating large language models' (LLMs) ability to follow complex, domain-specific formats, a crucial yet underexamined capability for their application as AI agents. Despite LLMs' advancements, existing benchmarks fail to assess their format-following proficiency adequately. FoFo fills this gap with a diverse range of real-world formats and instructions, developed through an AI-Human collaborative method. Our evaluation across both open-source (e.g., Llama 2, WizardLM) and closed-source (e.g., GPT-4, PALM2, Gemini) LLMs highlights three key findings: open-source models significantly lag behind closed-source ones in format adherence; LLMs' format-following performance is independent of their content generation quality; and LLMs' format proficiency varies across different domains. These insights suggest the need for specialized tuning for format-following skills and highlight FoFo's role in guiding the selection of domain-specific AI agents. FoFo is released here at https://github.com/SalesforceAIResearch/FoFo.

==> backups/backup.tex <==
\section{Introduction}

The exciting development of large language models (LLMs) in the past year~\citep{} implies their potentials on serving as the foundation model of AI assistants/agents in a variety of domains. 
People are getting increasingly optimistic that LLMs can at least help automate some steps in complicated tasks in various domains that currently require heavy human efforts, such as data analysis in the medical or legal world~\citep{}, code completion in the software industry~\citep{}, or simply serving as personalized assistants to finish daily chores such as making reservations/orders on line~\citep{}. 
In order for LLMs to successfully interact with humans, their capability of following human instructions is crucial~\citep{}. 
When it comes to serving as AI agents to accomplish middle steps in complicated tasks, instruction-following mostly falls into generating outputs that follow the exact formats given by humans.
For example, AI agents in Healthcare might be asked to organize medical records in HL7 Clinical Document Architecture (CDA) format~\citep{} for further processing. AI agents in marketing might be asked to generate KPI records following very company-specific formats to fit into existing evalution systems of different companies. 
Without the capacity to follow specific given formats, employing LLMs as AI agents wouldn't be practical.

However, existing evaluation benchmarks of LLMs are not specifically designed for evaluating the format-following capabilities of LLMs.  
On one hand, generic evaluation benchmarks such as alpaca-eval~\citep{} and MT-Bench~\citep{}, are mainly in the open question-answering/chatting format covering various knowledge domains such as math, coding and humanities, without taking the format-following capability of LLMs into consideration. 
Existing state-of-the-art LLMs from both the close-sourced and open-sourced world perform similarly well on them~\citep{}.
On the other hand, AI-agent evaluation benchmarks for specific environments, usually focus more on the final success rate of accomplishing test tasks in a specific environment. 
Since there are many factors that can affect final success rates, such as the model's grounding capability in the specific environment or the capacity of reasoning, the final success rates cannot directly reflect LLM's format-following capability.
Therefore, although we have found that LLMs performs significantly worse than humans as agents in quite some domains~\citep{}, we still don't know whether it is partially caused by format-following or whether improving LLMs on format-following can be a potential direction to further improve LLMs as AI agent foundation models.

To fill this gap, we propose to build a new format-following evaluation benchmark for LLMs. 
In this benchmark, we aim to cover diverse real-world domains that are likely to embrace LLMs as agents.
We also aim to build test examples that are as close to and as complicated as real-world use cases as possible, instead of testing LLMs on generic and simple format requirements without real-world context.
To achieve these two goals, we adopt a hierarchical approach to generate test cases. The generated results of each hierarchical step are evaluated and curated by human experts.
Specifically, we firstly generate and identify multiple real-world knowledge domains that are likely to benefit from LLMs, such as Healthcare, Finance, Technology and Software, etc. 
Then, for each domain we create a diverse sub-domain list,  identifying more specific sub-domains that can adopt LLMs to automatic their workflows.
Next, for each sub-domain, we generate domain-specific format list. 
Empirically we have found that through this hierarchical generation approach, we are able to collect more diverse format requirement since the domain -> sub-domain structure acts as a chain-of-thought process to encourage LLMs to traverse to more diverse and specific domains to propose  real-world format requirements.
Finally, given the domain -> sub-domain -> format meta-structure of every test example, we generate test prompts with complicated format requirements and specific real-world context.

After generating and human-curating the format-following benchmark, we evaluate various current top-performing LLMs on it.
Through our experiments and analysis, we have three main observations. 

1. Open sourced models significantly fall behind close-sourced models such as chatGPT~\citep{} and Google Gemini~\citep{} regarding to their fomat-following capability. Although on other more generic evaluation benchmarks such as Alpaca-eval, they all report similar performances. 
For example, wizard vs gpt3.

2. Among open sourced models, the rankings of their performance on format-following is also not consistent with their rankings on general evaluation benchmarks. 
For example, Mistral.
These two observations suggest that format-following capacity is independent of other capabilities of LLMs and might require tailored alignment fine-tuning with specific data beyond regular instruction-tuning that are widely used for training open-sourced LLMs ~\citep{}. 

3. The format-following capability of LLMs may vary a lot across different domains. We have found that even for two LLMs that give similar final accuracy on our benchmark, their accuracy on different domains can be very different.
For example,.
It indicates that format-following capacity is not generalizable across domains and our benchmark can potentially serve as guidance and probing tools for the choice of domain-specific AI agent foundation models.


\section{Related Work}


\textbf{Generic evaluation benchmarks.} There are multiple existing efforts that build evaluation data sets to try to assess LLMs' general problem-solving capability through conversations~\citep{}. 
Among them, MMLU data set~\citep{} is collected to measure knowledge and problem solving capabilities of LLMs in different knowledge domains such as elementary mathematics and US history. The performance of LLMs on MMLU is measured by the accuracy of their selected answers from multiple options.
Alpaca-eval~\citep{} and MT-bench~\citep{} on the other hand, collect open-ended questions accross different domains without providing concrete reference answers. They rely on LLMs such as GPT-4 to conduct automatic evaluations on the target LLM's answers. 
Except for these general benchmarks, there are also evaluation data sets specifically focusing on assess LLM answers truthfulness~\citep{}, helpfulness~\citep{} and safety~\citep{}.

\textbf{Instruction-following benchmarks.} In the past few months, the community starts to notice that the performance of existing and newly-emerging LLMs is saturating or ``overfitting'' on the generic benchmarks mentioned above~\citep{}.
However, the instruction-following capability, which is essential for applying LLMs into real-world use cases, are not specifically unveiled on these benchmarks.
Therefore, multiple instruction-following benchmarks are recently curated~\citep{}. 
These instruction-following benchmarks usually contain a small sub-set of test cases relevant to format following, such as generating data following JSON format, or following format requirements such as numbers of bullet points/paragraphs~\citep{}.
Compared to such format-following sub-sets that only covers a handful of generic formats such as JSON, our benchmark covers more diverse and domain-specific format requirements and each test example in our benchmark comes with complicated combined requirements and domain-specific context.
Therefore, we empirically find that our format-following benchmark is harder for existing LLMs and can unveil performance discrepancy across different domains  compared to the format-following sub sets in these benchmarks.


\section{Experiments}
\begin{table}[]
\centering
\resizebox{0.8\linewidth}{!}{% <-
\begin{tabular}{l|c} \hline
Attributes                               & Number \\ \hline
Domains                        & 10     \\ \hline
Subdomains                     & 50     \\ \hline
Data Formats                   & 248      \\ \hline
Test Prompts                   & 494    \\ \hline
Average Length of Test Prompts & 2908     \\ \hline
\end{tabular}
}
\caption{Data Statistics of our FoFo Benchmark.}
\label{tab:statistics}
\end{table}


\begin{table*}[] 
\begin{tabular}{l|c|c|c|c}\hline
%\begin{tabular}{p{0.25\textwidth}|p{0.75\textwidth}}  \hline
Model                        & Format Accuracy on FoFo&Avg. Length on FoFo       &  MT-Bench             & AlpacaEval\\\hline
Vicuna 13B V1.3              & 22.74                &2863                     &6.39                   &82.11      \\\hline
WizardLM 13B V1.1            & 27.00                  &3169                     &6.76                   &86.32      \\\hline
Vicuna 13B V1.5-16k          & 27.08                &3081                     &6.92                   &    -  \\\hline
Openchat V3.2-super          & 31.22                &3189                     &7.19                   &89.50      \\\hline
Llama 2 7B Chat              & 45.44                &4226                     &6.27                   &71.37      \\\hline
Mistral 7B Instruct V0.1     & 46.91                &5264                     &6.84                   &92.78      \\\hline
Llama 2 13B Chat             & 53.28                &4642                     &6.77                   &81.09      \\\hline
WizardLM 13B V1.2            & 63.54                &3511                     &7.2                    &89.17      \\\hline
%Mistral 8x7B                 &78.69                       &6943                         &8.3                    &94.78      \\\hline
%Openchat V3.5                & 72.28                &3600                     &7.81                   &  -    \\\hline
Zephyr 7B Beta               & 64.12                &6459                     &7.34                   &90.60      \\\hline\hline
GPT-3.5                      & 80.66                &4865                     &8.32                   &93.42      \\\hline
Gemini-pro                   & 80.25                &4434                     &        -               &79.66      \\\hline
palm2-text-bison-32k         & 83.72                &5371                     &     -                  &   -   \\\hline
GPT-4                        & 91.17                &3041                         &9.18                   &95.28      \\\hline
%GPT-4-Turbo                   & 94.87                &4140                         &     -                  &97.70      \\\hline
\end{tabular}
\caption{Main Results.}
\label{tab:main_result}
\end{table*}

\begin{figure*}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{sections/llama-mistral-2.png}
  \caption{A subfigure}
  \label{fig:llama-mistral}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{sections/wizardlm-zephyr-2.png}
  \caption{A subfigure}
  \label{fig:wizardlm-zephyr}
\end{subfigure}
\caption{A figure with two subfigures}
\label{fig:domain_analysis}
\end{figure*}


\begin{figure*}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{sections/llama-mistral-format.png}
  \caption{A subfigure}
  \label{fig:llama-mistral-format}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{sections/gpt-gemini-format.png}
  \caption{A subfigure}
  \label{fig:gpt-gemini-format}
\end{subfigure}
\caption{A figure with two subfigures}
\label{fig:fomat_analysis}
\end{figure*}

In this section, we present our empirical results and analysis of FoFo. The data  statistics of the FoFo benchmark are outlined in Table \ref{tab:statistics}. The average length of the test prompts is quantified in terms of characters to maintain consistency with the reporting standards established by AlpacaEval.

To verify FoFo's effectiveness on serving as a format-following benchmark of LLMs, we firstly select some top-performing LLMs~\citep{} from both the close-sourced and open-sourced world and evaluate them on FoFo.
Specifically, we are more interested in middle-sized LLMs that have shown similar performances to GPT-3.5 and GPT-4 on existing generic evaluation benchmarks such as MT-Bench and AlpacaEval because such LLMs are currently most widely-used.

To evaluate each open-sourced LLM, we employ its official prompt format to conduct generation given each test prompt in FoFo. During generation, we use sampling and set the temperature as 0.7 for all models for fair comparison. We also set the max new tokens to generate as 6144 for all models. After generation, we evaluate each LLM's format-following accuracy with GPT-4 as judge, as illustrated in Section 3.

\subsection{Main Results}
Table~\ref{tab:main_result} presents the format accuracy of all selected LLMs on FoFo. To better see the performance discrepancy of the same LLM on different benchmarks, we also list each LLM's performance on AlpacaEval and MT-Bench in Table~\ref{tab:main_result}.

The first observation we have from Table~\ref{tab:main_result} is that close-sourced models such as Gpt-3.5 and Gemini Pro (at lower part of the Table separated by double lines), significantly outperform open-sourced models in the upper part of the table. Close-sourced models all have above 80\% of format accuracy while open-source models reach only below 70\% of format accuracy. This performance gap is much more significant compared to their performance gap on existing generic benchmarks such as AlpacaEval.
For example, Mistral 7B Instruct V0.2 achieves 92.78\% of accuracy on AlpacaEval, comparable with GPT-3.5's 93.42\%. While it's format accuracy on FoFo is 46.91\%,  much lower compared to GPT-3.5's 80.66\%. Other open-sourced models also show similar performance pattern.

Second, we have found that performance of LLMs on FoFo is also not consistent with their performance on general evaluation benchmarks. 
For example, Openchat V3.2-super and WizardLM 13B V1.2 have similar performance on both AlpacaEval (around 89\%) and MT-Bench (around 7.2). While their format accuracy on FoFo has more than 30 points gap (31.22 vs 63.54). Gemini-pro has lower performance compared to GPT-3.5 on AlpacaEval while their format accuracy on FoFo is similar.

These two observations suggest that format-following capability is independent of other capabilities of LLMs reviewed by existing generic evaluation benchmarks. It  might require tailored alignment fine-tuning with specific data beyond regular instruction-tuning that are widely used for fine-tuning open-sourced LLMs.

We have also noticed in Table~\ref{tab:main_result} that the average length of responses on FoFo (around 4k) is generally larger compared with that on AlpacaEval (around 2k). 
This is due to the complexity of FoFo test prompts, as illustrated in the example prompt in Table~\ref{tab:prompt}. 
FoFo's test prompts usually combine many format requirements and ask for generating a complete and thorough document with a lot of domain-specific context.
Therefore, earlier models with 2k max sequence length, such as Vicuna 13B V1.3, might be at a disadvantage on FoFo. However, we also state that current LLMs' performance on FoFo is not capped by their max sequence length and a max sequence length of 5k is more than enough for achieving good accuracy on FoFo. Because GPT-4's average response length is 3041 and it's format accuracy is as high as 91.17\%.
%Length Analysis


\subsection{Result Analysis}
\noindent\textbf{Domain Analysis.} When analyzing empirical results on FoFo, we have also noticed that the format-following capability of LLMs may vary a lot across different domains. For two LLMs that give similar final accuracy on FoFo, their accuracy on different domains can be very different.  
Figure~\ref{fig:domain_analysis} shows two examples. Figure~\ref{fig:llama-mistral} shows the format-following accuracy comparison between Mistral 7B V0.2 and Llama 7B Chat across different domains. Their final performance on FoFo are very similar and both around 46\%. While we can see from  Figure~\ref{fig:llama-mistral} that Llama 7B Chat performs significantly worse on Scientific Research and Development domain and performs much better on Education domain. 
Similarly, WizardLM 13B V1.2 and Zephyr 7B Beta has similar final performance on FoFo (around 64\%) while Figure~\ref{fig:wizardlm-zephyr} shows they have their own expertise on different domains.
It indicates that format-following capacity is not generalizable across domains, possibly due to domain-specific formats such as HL7 Clinical Document Architecture (CDA) format in Healthcare. Our benchmark can potentially serve as guidance and probing tools for the choice of domain-specific AI agent foundation models.

\noindent\textbf{Format Analysis.}  As mentioned in Section 3, except domain-specific formats, FoFo also includes 5 general formats (JSON, XML, CSV, Markdown, and YAML.) and create test prompts with general formats and domain-specific context. 
After seeing the performance discrepancy across domains, we are also curious about whether LLMs have their own expertise on different genral formats. Therefore in Figure~\ref{fig:fomat_analysis}, we present the performance comparison of two LLMs achieving similar final accuracy across different general formats. 
Figure~\ref{fig:llama-mistral-format} shows that both Mistral 7B V0.2 and Llama 7B chat don't perform well on following csv format. While Mistral 7B V0.2 is good at json and markdown and Llama 7B chat expertizes in other two formats.
Figure~\ref{fig:llama-mistral-format} shows that both Gemini Pro and GPT-3.5 performs well on following YAML format and Gpt-3.5 is more specialized on JSON.

\noindent\textbf{Error Analysis.} Table \ref{tab:main_result} reveals that many open sourced LLMs underperform on our Format Following (FoFo) benchmark. To understand these shortcomings, we performed an error analysis focusing on Mistral 7B Instruct V0.1 as a representative model. We request human annotators to examine the explanations given by GPT-4 for the failure instances and categorize these reasons into the following groupings:

1. \textit{Incomplete Sections and Missing Information}: The model often neglects essential sections and details that the prompts mandate, spanning a variety of content areas such as methodological frameworks, data analyses, theoretical discussions, to name a few. This shortfall is especially pronounced in scientific contexts, as illustrated in Figure~\ref{fig:domain_analysis}, which depicts Mistral 7B V0.1's markedly inferior performance in scientific domains.

2. \textit{Incorrect Formatting and Structure}: Mistral 7B V0.1 truggles with adhering to specific formatting and structural guidelines, impacting diverse formats including JSON, CSV, Markdown, as well as domain-specific formats such as legal citations and academic referencing. Issues include improper syntax use, inaccurate data structure representations, and failure to follow document layout guidelines. Figure~\ref{fig:fomat_analysis} highlights the model's notably deficient capabilities in managing CSV, Markdown, and JSON formats.

%3. \textit{Lack of Detailed Content}: The model's responses often fall short in delivering the depth or specifics explicitly solicited in the prompts. This encompasses comprehensive analytical insights, thorough descriptions, complete argumentation, in-depth educational content, and domain-specific technical details. Consequently, the generated outputs tend to be superficial, failing to provide comprehensive information or utility. 4.. \textif{Failure to Adhere to Technical and Domain-specific Requirements}: The model's responses inconsistently capture the technical nuances or meet the specific requirements of the prompts, including programming script formats, legal brief components, and detailed scientific data or analysis.

3. \textit{Lack of Detailed Content}: The model often fails to provide the depth or specifics required by the prompts, leading to outputs that are superficial and lack comprehensive information or utility. Despite requests for detailed analytical insights, exhaustive descriptions, and domain-specific technical details, the model's responses miss capturing the technical subtleties or fulfilling the specialized requirements, affecting a range of formats from programming scripts to legal brief components and detailed scientific analyses.

4. \textit{Inaccurate Simulation or Conceptualization}: For prompts requesting imaginative or conceptual examples, the model often provides unrealistic or oversimplified constructs, failing to effectively illustrate the intended concepts.

\noindent\textbf{Human Evaluation Alignment.} To assess the effectiveness of utilizing GPT-4 as an evaluation tool, we random sampled 100 prompts from our benchmark and generated responses using the Mistral 7B model. Subsequently, GPT-4 was employed to annotate these prompt-response pairs. To validate the accuracy of GPT-4's annotations, we engaged five human experts to evaluate the correctness of GPT-4's evaluations and analyzed the alignment between human annotators and the GPT-4 evaluator. Our findings revealed that for 84 out of the 100 prompts, the evaluations by GPT-4 were in agreement with those of the human experts, yielding an alignment rate of 84\%. A closer examination was conducted on the 16 instances where GPT-4's evaluations diverged from human judgment. It was observed that all these discrepancies were instances of false positives, indicating scenarios where the model's outputs failed to adhere to specific format requirements, yet were overlooked by GPT-4. For example, one prompt required the inclusion of an address, which was absent in the model's output. Another prompt necessitated a numerical value in percentage format, which was not provided. Additional errors included the generation of an insufficient number of examples, omission of a required section, and the introduction of non-existent tags. Consequently, these findings suggest that the actual performance of the models might be lower than what is reported by GPT-4's evaluations. 

Taking human evaluations as a benchmark, we infer that the real performance of the models could be approximately 16\% lower than the figures presented in Table~\ref{tab:main_result}. For example, the accuracy of the Mistral 7B Instruct V0.2 model, as evaluated by GPT-4, stands at 46.91\%, but its actual performance is estimated to be around 39.4\%. While employing GPT-4 as an evaluator has its limitations, it significantly reduces the workload associated with human evaluation and provides insights into the comparative performance of different models. For instance, our benchmark indicates that the Llama 2 13B Chat model outperforms Llama 2 7B Chat a lot.

\noindent\textbf{Cost Analysis} In this study, we utilize GPT-4 for both the construction of our benchmark and the evaluation of large-scale language models (LLMs). This approach incurs certain costs associated with utilizing the GPT-4 API. The cost is determined by the number of tokens in both the input and output, with pricing set at \$0.03 per 1,000 input tokens and \$0.06 per 1,000 output tokens\footnote{\url{https://openai.com/pricing}}. Given that one token approximately equates to four characters of common English text according to OpenAI's guidelines\footnote{\url{https://platform.openai.com/tokenizer}}, we can estimate the average number of tokens based on the character count.

%In constructing our benchmark, we identified two primary steps that incur costs associated with utilizing the GPT-4 API: the generation of domain-specific data formats, and the creation of test prompts. The process for generating data formats, as delineated in Algorithm~\ref{alg:data_formats}, reveals that the mean length of input characters is 518, approximately translating to 130 tokens in GPT-4 terminology. The corresponding average output character length stands at 1737, or equivalently, around 434 GPT-4 tokens. This results in an average cost calculation of \$0.03 * 0.13 + \$0.06 * 0.434 = \$0.03 per prompt. Given our methodology involves invoking this prompt 25 times across various domains and subdomains (5 domains * 5 subdomains), the total expenditure for this phase is computed to be \$0.75.

In the process of developing our benchmark, the primary expenditure arises during the creation of test prompts, as detailed in Algorithm~\ref{alg:prompts}. Analysis reveals that the mean length of input characters is 818, translating to approximately 205 GPT-4 tokens. Conversely, the output character count averages at 2908, equivalent to about 727 GPT-4 tokens. This setup yields an average cost per prompt of \$0.03 * 0.205 (for the input) + \$0.06 * 0.727 (for the output), amounting to \$0.05. Considering the necessity to craft 500 such prompts, the aggregate cost allocated for the generation of test prompts stands at \$25.

In our evaluation of various LLMs using GPT-4, the inputs consist of three components as detailed in Appendix \ref{app:eval_temp}: the length of the evaluation template, the length of the test prompt, and the length of the model outputs. The evaluation template has a character length of 1,594. As indicated in Table~\ref{tab:statistics}, the average character length of the test prompts is 2,908. By referring to Table~\ref{tab:main_result}, we deduce the average character length of the outputs to be 4,163. Consequently, the average input character length for evaluation purposes totals 8,665, equivalent to approximately 2,166 tokens for GPT-4. This results in an average input cost of: \$0.03 * 2.166 = \$0.065. For the outputs, the average character length during evaluation is 1,098, translating to roughly 275 tokens for GPT-4. This leads to an average output cost of: \$0.06 * 0.275 = \$0.0165. Therefore, the average cost of evaluating one LLM using a single prompt stands at \$0.0815. The entire Format Following (FoFo) benchmark comprises 494 prompts, culminating in a total evaluation cost of approximately \$40 for one LLM across the entire benchmark. In future endeavors, we are considering the adoption of GPT-4-Turbo for evaluation purposes to further mitigate costs.

\subsection{Ablations}
\noindent\textbf{Ablation on removing ``sub-domains'' from the prompt generation method.}
As illustrated in Section 3, our hierarchical test prompt generation method firstly create a diverse set of domains and then a diverse sub-domain list for each domain.
We state that this domain -> sub-domain structure is necessary for guaranteeing the diversity and coverage of the generated formats.  
We have used Algorithm 1 but without the sub-domain labels to generate the same number of formats for each domain as FoFo. We found that this variation fails to cover some important categories of formats under some domains and the format requirements generated by this variation can be quite monotone. Case study is presented in Appendix~\ref{}.

\noindent\textbf{Comparison with IfEval.} As mentioned in Algorithm 2, when generating each test prompt of FoFo, we prompt GPT-4 to make the output a detailed and complicated content generation task with specific format configurations.
As a result, each test prompt of FoFo contains many complicated domain-specific format requirements, as shown in Table~\ref{tab:prompt}.
This is one of the main differences that FoFo has compared to other instruction-following benchmarks such as IfEval. Although IfEval has a sub-set of prompts that test the format-following capability of LLMs, they are domain-agnostic and contain only digital number of format configurations. 
We evaluate representative open-sourced and close-sourced LLMs on IfEval's format-following sub-set too and find that they all achieve much higher accuracy on IfEval's sub-set compared to on FoFo, as shown in Table~\ref{} in Appendix. 
It indicates that FoFo is not only the first domain-specific format-following benchmark, but also a much harder one compared to current generic format-following test sets.

\noindent\textbf{Content accuracy analysis.} As illustrated in Section 3.2, for now we only evaluate whether a LLM correctly follows the format requirements given by FoFo test prompts. One may also be curious about LLMs' content accuracy on FoFo. Therefore we also modified our judge prompt to evaluate whether the generated content is correct given each FoFo test prompt, regardless of the format accuracy. We present this result in Table~\ref{} in Appendix.  It shows the LLMs' content accuracy is in general higher than their corresponding format accuracy.



\subsection{List of domain and agents}
\begin{enumerate}
    \item \textbf{Healthcare}: AI assists in diagnostics, treatment personalization, drug development, and patient care management, revolutionizing the speed and efficacy of healthcare services.
    \begin{enumerate}
     \item Medical Diagnostics: AI agents can analyze medical data such as patient history, symptoms, and test results to assist healthcare professionals in diagnosing illnesses and diseases.
    \item Medical Treatment: AI agents can suggest personalized treatment plans by analyzing patient data, medical literature, and clinical guidelines, aiding healthcare professionals in making informed decisions.
    \item Patient Care Management: AI agents can monitor and analyze patient data in real-time to provide personalized care plans, detect anomalies, and alert healthcare providers about potential risks or changes in patient conditions.
    \item Clinical Trial Analysis: AI agents can assist in the analysis of clinical trial data, identifying trends, predicting outcomes, and contributing to the development of new treatments and therapies.
    \item Pharmaceuticals: AI agents can aid in drug discovery, screening potential molecules, predicting their efficacy, and optimizing drug formulations, ultimately accelerating the research and development process.
    \end{enumerate}

\item \textbf{Finance}: Leveraging AI for fraud detection, algorithmic trading, personalized financial advice, and risk management is transforming the finance industry.
    \begin{enumerate}
     \item Fraud Detection: AI systems can analyze transaction patterns in real-time to detect anomalous behavior that may indicate fraud. They can consider historical and current transaction data, customer profiles, and typical user behaviors to identify potential fraud.
    \item Algorithm Trading: AI agents can process vast amounts of financial market data, including price changes, news feeds, and economic indicators, to make automated trading decisions quickly and efficiently.
    \item Personalized Financial Advice: AI leverages data analytics and machine learning to offer customized investment strategies and financial planning tailored to individual goals and risk profiles.
    \item Risk management: AI provides sophisticated predictive models and simulations to identify, assess, and mitigate financial risks in portfolio management and lending processes.
    \item Regulatory Compliance: AI agents can assist financial institutions by continuously monitoring and ensuring compliance with relevant regulations. They can analyze transactions, communications, and other activities to detect any potential breaches or non-compliant behavior.
    \end{enumerate}
    
\item \textbf{Technology and Software}: Automation of coding, testing, data analysis, system design, and development processes is making technology development faster and more efficient.
    \begin{enumerate}
    \item Web Design: AI agents can assist in creating website layouts, suggesting design elements that align with best practices, and generating code for those designs. They may also personalize the user experience based on visitor behavior.
    \item Programming: AI can support developers by automating repetitive coding tasks, suggesting code completions, and providing real-time debugging assistance.
    \item UI/UX Design: AI tools can help optimize user interfaces by analyzing user interactions and providing insights on how to improve the user experience. AI could generate heatmaps, user journey maps, and even suggest improvements to the UI elements.
    \item Data Analysis: AI agents can process large datasets to identify trends, perform predictive analysis, or generate insights that can drive decision-making. AI tools can be used for analyzing user behavior, system performance, or market trends.
    \item Testing: AI can enhance software testing by automating test case generation, executing tests, identifying bugs, and learning from previous iterations to improve test coverage.
    \end{enumerate}
    
\item \textbf{Commerce and Manufacturing}: AI in commerce and manufacturing is reshaping how businesses interact with customers, manage their supply chain, and optimize their production processes.
    \begin{enumerate}
    \item E-commerce Personalization: AI agents analyze customer behavior, purchase history, and preferences to deliver tailored shopping experiences. They can recommend products, customize search results, and offer personalized discounts, enhancing customer engagement and sales conversion rates.
    \item Manufacturing Process Optimization: In manufacturing, AI agents are applied to optimize production processes by analyzing machine performance, predicting maintenance, and increasing operational efficiency. They schedule machinery maintenance to minimize downtime, calculate the most efficient production paths, and ensure optimal resource allocation. 
    \item Inventory and Supply Chain Management: AI agents improve inventory control by predicting stock levels, automating reordering processes, and optimizing warehouse layouts. For supply chain management, they analyze logistics data, track shipments in real-time, and forecast demand to minimize stockouts and overstocking.
    \item Quality Control: AI is utilized in quality assurance processes to identify defects in products using computer vision and machine learning algorithms. These agents automate inspections, analyze product data across various stages of manufacturing, and reduce human error rate associated with manual inspection.
    \item Smart Logistics and Route Optimization: AI optimizes delivery routes, predicts transit times, and manages fleet operations to enhance supply chain efficiency. It analyzes traffic data, weather conditions, and delivery schedules to determine the best routes, adjust plans in real-time, and optimize last-mile delivery.
    \end{enumerate}

\item \textbf{Customer Relationship Management (CRM)}: AI in customer relationship management (CRM) enhances customer service, predicts sales, streamlines recruitment, improves project management, and analyzes sentiment to improve overall customer satisfaction and business success.
    \begin{enumerate}
    \item Customer Service: AI agents can assist in handling customer inquiries, providing accurate and prompt responses, improving customer satisfaction.
    \item Sales Forecasting: AI agents can analyze historical sales data, market trends, and customer behavior to predict future sales and help businesses make informed decisions.
    \item Recruitment Assistants: AI agents can streamline the recruitment process by analyzing resumes, conducting initial screenings, and identifying qualified candidates based on predefined criteria, saving time and effort for HR professionals.
    \item Project Management: AI agents can assist in project planning, resource allocation, and task management by analyzing historical project data, identifying potential risks, and suggesting optimal project timelines and resource allocations.
    \item Lead Scoring: AI algorithms can prioritize leads based on their likelihood to convert, analyzing engagement patterns, demographics, and previous interactions to score and rank prospects, enabling sales teams to focus on the most promising opportunities.
    \end{enumerate}
    
\item \textbf{Marketing}: AI's ability to analyze consumer data and optimize advertising campaigns is revolutionizing how products and services are marketed to audiences.
    \begin{enumerate}
    \item Consumer Behavior Analysis: AI can analyze large volumes of consumer data to identify patterns and trends in purchasing behavior, enabling marketers to understand their target audience better.
    \item Advertising Campaign Optimization: AI algorithms can optimize ad campaigns in real-time by analyzing performance data and adjusting parameters such as placement, content, and audience targeting.
    \item Content Curation and Creation: AI can assist in generating and curating content for various marketing channels. It can analyze engagement data to suggest topics that resonate with audiences or even create initial drafts of content such as social media posts, blog articles, or personalized email messages.
    \item Social Media Management: AI tools can help manage and optimize a company's presence on social media platforms. They can schedule posts, suggest content, engage with followers by replying to comments, and analyze social media analytics to refine strategies.
    \item Search Engine Optimization (SEO): AI can analyze search data, suggest keywords, optimize website content, and track competitor SEO strategies to improve search engine rankings. 
    \end{enumerate}
    
\item \textbf{Scientific Research and Development}: AI boosts the speed and capacity for analyzing data, simulating environments, and expediting discoveries in fields like climate science, physics, and genetics.
    \begin{enumerate}
    \item Mathematical Research: AI can assist in solving complex mathematical problems, identifying patterns in large datasets, and even contributing to the development of new mathematical theories.
    \item Physics: AI is playing a crucial role in analyzing experimental data, simulating physical phenomena, and helping physicists in theoretical developments.
    \item Chemistry and Biological Sciences: In the domains of chemistry and biological sciences, AI aids in drug discovery, accelerates genome analysis, and enables the prediction of molecular behavior, thereby transforming research and personalized medicine.
    \item Environmental Sciences and Climate Change: AI's predictive power can be leveraged to understand and combat climate change and manage natural resources more effectively.
    \item Space Exploration: AI contributes significantly to processing astronomical data, guiding autonomous spacecraft, and even aiding in the search for extraterrestrial life.
    \end{enumerate}
    
\item \textbf{Education}: Adaptive learning platforms, AI tutors, and automated grading systems are personalizing and enhancing education at both individual and institutional levels.
    \begin{enumerate}
    \item Adaptive Learning Platforms: AI-driven learning platforms can adjust the content, pace, and learning style based on individual student performance and engagement, tailoring the educational process to each student's needs.
    \item Intelligent Tutoring Systems: AI-powered tutoring systems can simulate one-on-one interaction with a human tutor, offering students immediate feedback and tailored instruction.
    \item Automated Grading Systems: AI can evaluate and grade student assignments and exams, saving educators time and providing students with faster feedback.
    \item Education Data Analysis: AI can analyze educational data at scale to uncover insights that help educators understand learning patterns, predict student performance, and improve teaching strategies.
    \item Language Learning: AI-powered language learning apps use speech recognition and natural language processing to provide learners with real-time pronunciation feedback, vocabulary exercises, and conversational practice.
    \end{enumerate}
    
\item \textbf{Legal}: AI can help with document analysis, legal research, due diligence, and even in predicting legal outcomes.
    \begin{enumerate}
    \item Contract Review and Analysis: AI agents can examine large volumes of contracts to identify clauses, assess risks, and ensure that agreements comply with relevant laws and regulations, thereby streamlining the contract vetting process for legal professionals.
    \item Legal Document Automation: AI can automate the drafting of legal documents based on predefined templates and rules, reducing manual efforts and the likelihood of human error in routine paperwork like wills, leases, and compliance forms.
    \item Legal Research: AI can quickly sift through millions of legal documents, case laws, and statutes to find relevant precedents and interpretations, saving time for lawyers and improving the legal argumentation process.
    \item Predictive Legal Analytics: These AI systems can analyze past legal outcomes to predict future rulings, helping attorneys to strategize more effectively and anticipate case results.
    \item Intellectual Property (IP) Management: AI can assist in the management and analysis of IP portfolios by monitoring patents, trademarks, and copyrights, identifying infringement risks, and suggesting opportunities for IP development.
    \end{enumerate}
    
\item \textbf{Arts and Entertainment}:
    \begin{enumerate}
    \item Music Composition: AI can generate new musical pieces by learning from vast collections of music styles and genres, offering artists novel composition tools and inspirations.
    \item Film Scriptwriting: AI agents can analyze successful screenplays to help scriptwriters create engaging story arcs, dialogues, and character development, streamlining the writing process.
    \item Visual Art Creation: Utilizing machine learning, AI can craft original artworks by analyzing artistic techniques and historical styles, providing new forms of digital art for creators and consumers.
    \item Video Game Development: AI can design complex in-game behaviors and environments, adapt difficulty based on player skill levels, and create personalized gaming experiences.
    \item Sports Analytics and Performance: AI can process player statistics, game footage, and biometric data to provide coaches with tactical insights and personalized athlete training regimens.
    \end{enumerate}
\end{enumerate}








\begin{table*}
\begin{tabular}{p{0.1\textwidth}p{0.2\textwidth}p{0.7\textwidth}}
Domain                                                  & Sub Domains                               & Description      \\
\multirow{5}{*}{Healthcare}                             & Medical Diagnostics                       & AI agents can analyze medical data such as patient history, symptoms, and test results to assist healthcare professionals in diagnosing illnesses and diseases.                                                                                                                                                            \\
 & Medical Treatment                         & AI agents can suggest personalized treatment plans by analyzing patient data, medical literature, and clinical guidelines, aiding healthcare professionals in making informed decisions.                                                                                                                                   \\
& Patient Care Management                   & AI agents can monitor and analyze patient data in real-time to provide personalized care plans, detect anomalies, and alert healthcare providers about potential risks or changes in patient conditions.                                                                                                                   \\
 & Clinical Trial Analysis                   & AI agents can assist in the analysis of clinical trial data, identifying trends, predicting outcomes, and contributing to the development of new treatments and therapies.                                                                                                                                                 \\
& Pharmaceuticals                           & AI agents can aid in drug discovery, screening potential molecules, predicting their efficacy, and optimizing drug formulations, ultimately accelerating the research and development process.                                                                                                                             \\
\multirow{5}{*}{Finance}                                & Fraud Detection                           & AI systems can analyze transaction patterns in real-time to detect anomalous behavior that may indicate fraud. They can consider historical and current transaction data, customer profiles, and typical user behaviors to identify potential fraud.                                                                       \\
& Algorithm Trading                         & AI agents can process vast amounts of financial market data, including price changes, news feeds, and economic indicators, to make automated trading decisions quickly and efficiently.                                                                                                                                    \\
& Personalized Financial Advice             & AI leverages data analytics and machine learning to offer customized investment strategies and financial planning tailored to individual goals and risk profiles.                                                                                                                                                          \\
& Risk management                           & AI provides sophisticated predictive models and simulations to identify, assess, and mitigate financial risks in portfolio management and lending processes.                                                                                                                                                               \\
& Regulatory Compliance                     & AI agents can assist financial institutions by continuously monitoring and ensuring compliance with relevant regulations. They can analyze transactions, communications, and other activities to detect any potential breaches or non-compliant behavior.                                                                  \\
\multirow{5}{*}{Technology and Software}                & Web Design                                & AI agents can assist in creating website layouts, suggesting design elements that align with best practices, and generating code for those designs. They may also personalize the user experience based on visitor behavior.                                                                                               \\
& Programming                               & AI can support developers by automating repetitive coding tasks, suggesting code completions, and providing real-time debugging assistance.                                                                                                                                                                                \\
& UI/UX Design                              & AI tools can help optimize user interfaces by analyzing user interactions and providing insights on how to improve the user experience. AI could generate heatmaps, user journey maps, and even suggest improvements to the UI elements.                                                                                   \\
 & Data Analysis                             & AI agents can process large datasets to identify trends, perform predictive analysis, or generate insights that can drive decision-making. AI tools can be used for analyzing user behavior, system performance, or market trends.    \\                     & Testing                                   & AI can enhance software testing by automating test case generation, executing tests, identifying bugs, and learning from previous iterations to improve test coverage.                                                                                                                                                     \\
\multirow{5}{*}{Commerce and Manufacturing}             & E-commerce Personalization                & AI agents analyze customer behavior, purchase history, and preferences to deliver tailored shopping experiences. They can recommend products, customize search results, and offer personalized discounts, enhancing customer engagement and sales conversion rates.                                                        \\
& Manufacturing Process Optimization        & In manufacturing, AI agents are applied to optimize production processes by analyzing machine performance, predicting maintenance, and increasing operational efficiency. They schedule machinery maintenance to minimize downtime, calculate the most efficient production paths, and ensure optimal resource allocation. \\
& Inventory and Supply Chain Management     & AI agents improve inventory control by predicting stock levels, automating reordering processes, and optimizing warehouse layouts. For supply chain management, they analyze logistics data, track shipments in real-time, and forecast demand to minimize stockouts and overstocking.                                     \\
 & Quality Control                           & AI is utilized in quality assurance processes to identify defects in products using computer vision and machine learning algorithms. These agents automate inspections, analyze product data across various stages of manufacturing, and reduce human error rate associated with manual inspection.                        \\
& Smart Logistics and Route Optimization    & AI optimizes delivery routes, predicts transit times, and manages fleet operations to enhance supply chain efficiency. It analyzes traffic data, weather conditions, and delivery schedules to determine the best routes, adjust plans in real-time, and optimize last-mile delivery.                                      \\
\multirow{5}{*}{Customer Relationship Management (CRM)} & Customer Service                          & AI agents can assist in handling customer inquiries, providing accurate and prompt responses, improving customer satisfaction.                                                                                                                                                                                             \\
& Sales Forecasting                         & AI agents can analyze historical sales data, market trends, and customer behavior to predict future sales and help businesses make informed decisions.                                                                                                                                                                     \\
 & Recruitment Assistants                    & AI agents can streamline the recruitment process by analyzing resumes, conducting initial screenings, and identifying qualified candidates based on predefined criteria, saving time and effort for HR professionals.                                                                                                      \\
& Project Management                        & AI agents can assist in project planning, resource allocation, and task management by analyzing historical project data, identifying potential risks, and suggesting optimal project timelines and resource allocations.                                                                                                   \\
& Lead Scoring                              & AI algorithms can prioritize leads based on their likelihood to convert, analyzing engagement patterns, demographics, and previous interactions to score and rank prospects, enabling sales teams to focus on the most promising opportunities.                                                                            \\
\multirow{5}{*}{Marketing}                              & Consumer Behavior Analysis                & AI can analyze large volumes of consumer data to identify patterns and trends in purchasing behavior, enabling marketers to understand their target audience better.                                                                                                                                                       \\
& Advertising Campaign Optimization         & AI algorithms can optimize ad campaigns in real-time by analyzing performance data and adjusting parameters such as placement, content, and audience targeting.                                                                                                                                                            \\
& Content Curation and Creation             & AI can assist in generating and curating content for various marketing channels. It can analyze engagement data to suggest topics that resonate with audiences or even create initial drafts of content such as social media posts, blog articles, or personalized email messages.                                         \\
& Social Media Management                   & AI tools can help manage and optimize a company's presence on social media platforms. They can schedule posts, suggest content, engage with followers by replying to comments, and analyze social media analytics to refine strategies.                                                                                    \\
 & Search Engine Optimization (SEO)          & AI can analyze search data, suggest keywords, optimize website content, and track competitor SEO strategies to improve search engine rankings.                                                                                                                                                                             \\
\multirow{5}{*}{Scientific Research and Development}    & Mathematical Research                     & AI can assist in solving complex mathematical problems, identifying patterns in large datasets, and even contributing to the development of new mathematical theories.                                                                                                                                                     \\
& Physics                                   & AI is playing a crucial role in analyzing experimental data, simulating physical phenomena, and helping physicists in theoretical developments.                                                                                                                                                                            \\
& Chemistry and Biological Sciences         & In the domains of chemistry and biological sciences, AI aids in drug discovery, accelerates genome analysis, and enables the prediction of molecular behavior, thereby transforming research and personalized medicine.                                                                                                    \\
& Environmental Sciences and Climate Change & AI's predictive power can be leveraged to understand and combat climate change and manage natural resources more effectively.                                                                                                                                                                                              \\
& Space Exploration                         & AI contributes significantly to processing astronomical data, guiding autonomous spacecraft, and even aiding in the search for extraterrestrial life.                                                                                                                                                                      \\
\multirow{5}{*}{Education}                              & Adaptive Learning Platforms               & AI-driven learning platforms can adjust the content, pace, and learning style based on individual student performance and engagement, tailoring the educational process to each student's needs.                                                                                                                           \\
& Intelligent Tutoring Systems              & AI-powered tutoring systems can simulate one-on-one interaction with a human tutor, offering students immediate feedback and tailored instruction.                                                                                                                                                                         \\
 & Automated Grading Systems                 & AI can evaluate and grade student assignments and exams, saving educators time and providing students with faster feedback.                                                                                                                                                                                                \\
& Education Data Analysis                   & AI can analyze educational data at scale to uncover insights that help educators understand learning patterns, predict student performance, and improve teaching strategies.                                                                                                                                               \\
& Language Learning                         & AI-powered language learning apps use speech recognition and natural language processing to provide learners with real-time pronunciation feedback, vocabulary exercises, and conversational practice.                                                                                                                     \\
\multirow{5}{*}{Legal}                                  & Contract Review and Analysis              & AI agents can examine large volumes of contracts to identify clauses, assess risks, and ensure that agreements comply with relevant laws and regulations, thereby streamlining the contract vetting process for legal professionals.                                                                                       \\
& Legal Document Automation                 & AI can automate the drafting of legal documents based on predefined templates and rules, reducing manual efforts and the likelihood of human error in routine paperwork like wills, leases, and compliance forms.                                                                                                          \\
& Legal Research                            & AI can quickly sift through millions of legal documents, case laws, and statutes to find relevant precedents and interpretations, saving time for lawyers and improving the legal argumentation process.                                                                                                                   \\
& Predictive Legal Analytics                & These AI systems can analyze past legal outcomes to predict future rulings, helping attorneys to strategize more effectively and anticipate case results.                                                                                                                                                                  \\
& Intellectual Property (IP) Management     & AI can assist in the management and analysis of IP portfolios by monitoring patents, trademarks, and copyrights, identifying infringement risks, and suggesting opportunities for IP development.                                                                                                                          \\
\multirow{5}{*}{Arts and Entertainment}                 & Music Composition                         & AI can generate new musical pieces by learning from vast collections of music styles and genres, offering artists novel composition tools and inspirations.                                                                                                                                                                \\
& Film Scriptwriting                        & AI agents can analyze successful screenplays to help scriptwriters create engaging story arcs, dialogues, and character development, streamlining the writing process.                                                                                                                                                     \\
& Visual Art Creation                       & Utilizing machine learning, AI can craft original artworks by analyzing artistic techniques and historical styles, providing new forms of digital art for creators and consumers.                                                                                                                                          \\
& Video Game Development                    & AI can design complex in-game behaviors and environments, adapt difficulty based on player skill levels, and create personalized gaming experiences.                                                                                                                                                                       \\
 & Sports Analytics and Performance          & AI can process player statistics, game footage, and biometric data to provide coaches with tactical insights and personalized athlete training regimens.                                                                                           \end{tabular}                                                               
\end{table*}








Prompt Example:

Generate a comprehensive medical prescription for a 55-year-old patient diagnosed with Type 2 Diabetes Mellitus and Hypertension. The prescription should adhere to the Prescription Format Standard (PFS-2021) specified below:

1. Patient Information:
   - Full Name: John A. Doe
   - Age: 55
   - Sex: Male
   - Weight: 90 kg
   - Height: 175 cm
   - Allergies: Penicillin

2. Diagnosis:
   - Primary Diagnosis: Type 2 Diabetes Mellitus
   - Secondary Diagnosis: Hypertension

3. Prescription Date: [Today's date]

4. Medications:
   - Itemize each medication with the following details:
     a. Generic Name
     b. Brand Name (if applicable)
     c. Strength
     d. Form (tablet, capsule, injection, etc.)
     e. Dosage
     f. Administration route (oral, IV, etc.)
     g. Frequency and duration of intake
     h. Special instructions (e.g., taken with food, on an empty stomach, etc.)
     
5. Lifestyle Recommendations:
   - Include at least three recommendations relevant to the diagnosis.

6. Lab Tests:
   - List any lab tests required before the next visit.

7. Refills:
   - Specify the number of refills for each medication.

8. Physician Information:
   - Full Name: Dr. Emily R. Smith
   - Medical License Number: 123456
   - Specialty: Endocrinology
   - Contact Number: (555) 123-4567
   - Clinic Address: 123 Healthy Way, Wellness City, HC 67890

9. Follow-up:
   - Date and Time for next appointment (if applicable).

Ensure the following PFS-2021 configuration requirements are met:
- Use clear, legible font, Arial Size 11
- Align patient information and diagnosis to the left
- Medications should be listed in a table format with clear column headings
- Lifestyle recommendations should be in bullet points
- Lab Tests and Refills should be in separate, clearly labeled sections
- Follow-ups should be highlighted

Please improvise any additional details required that have not been explicitly provided, ensuring the generated content aligns with the patient's condition and common medical practice.










\begin{table*}[] 
\centering
\resizebox{\linewidth}{!}{% <-
\begin{tabular}{
  llcccc
}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{Model}} & \multicolumn{2}{c}{\formatfollowing~({\dataname})} & \multicolumn{2}{c}{{\contentfollowing}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6}
&  & {Format Accuracy} & {Avg. Length} & {MT-Bench} & {AlpacaEval} \\
\midrule
% \multicolumn{5}{c}{Open-sourced LLMs} \\
\midrule
\multirow{9}{*}{\rotatebox{90}{Open-source}} & Vicuna 13B V1.3~\citep{chiang2023vicuna} & 22.74 & 2863 & 6.39 & 82.11 \\
& WizardLM 13B V1.1~\citep{xu2023wizardlm} & 27.00 & 3169 & 6.76 & 86.32 \\
& Vicuna 13B V1.5-16k~\citep{chiang2023vicuna} & 27.08 & 3081 & 6.92 & - \\
& Openchat V3.2-super~\citep{wang2023openchat} & 31.22 & 3189  &7.19 & 89.50 \\
& Llama 2 7B Chat~\citep{touvron2023llama} & 45.44 & 4226 &6.27 &71.37  \\
& Mistral 7B Instruct V0.1~\citep{jiang2023mistral} & 46.91 &5264 &6.84 &92.78 \\
& Llama 2 13B Chat~\citep{touvron2023llama} & 53.28 &4642 & 6.77 &81.09 \\
& WizardLM 13B V1.2~\citep{xu2023wizardlm} & 63.54 &3511 &7.2 &89.17 \\
%Mistral 8x7B &78.69  &6943 &8.3 &94.78  \\
%Openchat V3.5 & 72.28 &3600 &7.81 &  -  \\
& Zephyr 7B Beta~\citep{tunstall2023zephyr} & 64.12 &6459 &7.34 &90.60  \\
\midrule
% \multicolumn{5}{c}{Closed-sourced LLMs} \\
\midrule
\multirow{4}{*}{\rotatebox{90}{Closed-sour.}} & GPT-3.5~\citep{openai2023chatgpt} & 80.66 & 4865 & 8.32 & 93.42 \\
& Gemini Pro~\citep{google2023gemini} & 80.25 & 4434 & - & 79.66 \\
& PaLM 2 for Text 32k~\citep{anil2023palm}  & 83.72  &5371 & - &   -   \\
& GPT-4~\citep{openai2023gpt4} & 91.17 & 3041 & 9.18 & 95.28 \\
\bottomrule
\end{tabular}
}
\caption{Main Results. \jiangshu{The source of the models can be found in Appendix~\ref{app:eval_models}.}}
\label{tab:main_result}
\end{table*}

==> backups/domain_specific_data_format_backup.tex <==
\onecolumn
\begin{longtable}{>{\raggedright\arraybackslash}p{0.16\linewidth}
                  >{\raggedright\arraybackslash}p{0.22\linewidth}
                  >{\raggedright\arraybackslash}p{0.41\linewidth}}
\toprule
      Domain & Subdomain & Dataformat \\ \midrule
\midrule
\endfirsthead

\toprule
      Domain & Subdomain & Dataformat \\ \midrule
\midrule
\endhead

\midrule
\multicolumn{3}{r}{{Continued on next page}} \\ \bottomrule
\endfoot

\bottomrule
\endlastfoot

\multirow{30}{*}{Healthcare}   & {Medical Diagnostics}  & \parbox[t]{\linewidth}{
    ICD-10 format (International Classification of Diseases 10th Revision); \\ 
    CAP format (College of American Pathologists protocol); \\
    DICOM SR (Structured Report); \\
    HL7 CDA (Health Level Seven Clinical Document Architecture)
} \\
\cmidrule{2-3}
 & {Medical Treatment}     & \parbox[t]{\linewidth}{
 Medical Reports; \\
 Prescription Formats; \\
 SOAP Notes;  \\ 
 Discharge Summary; \\
 Clinical Trial Protocols }    \\
 \cmidrule{2-3}
& Patient Care   Management       & \parbox[t]{\linewidth}{
Electronic Health Record (EHR) Format; \\
Discharge Summary Format;\\
Clinical Trial Report Format; \\
Prescription Format; \\
Medical Coding and Billing Statement Format }  \\
\cmidrule{2-3}
 & Clinical Trial   Analysis       & \parbox[t]{\linewidth}{
 Clinical Study Report (CSR); \\
 Clinical Trial   Protocol; \\
 Patient Reported Outcomes (PRO); \\
 Patient Data Report (PDR); \\
 Adverse Event Report (AER) }\\
 \cmidrule{2-3}
& Pharmaceuticals                 & \parbox[t]{\linewidth}{
RxNorm Format; \\
HL7 (Health Level 7) Format; \\
ICD-10   Format; \\
LOINC Format; \\
Fast Healthcare Interoperability Resources (FHIR)   Format} \\ 
\midrule
\multirow{17}{*}{Finance}                   & Fraud Detection                 & \parbox[t]{\linewidth}{
Compromised Account Report Format; \\
Credit Card   Fraud Alert Format; \\
Investment Fraud Detection Report; \\
Loan Fraud Report  Format; \\
Insurance Fraud Detection Report} \\
\cmidrule{2-3}
 & Algorithm Trading               & \parbox[t]{\linewidth}{
 FIX Protocol Message; \\
 Standard Portfolio Analysis   of Risk (SPAN) Data; \\
 Thomson Reuters EIKON data; \\
 Bloomberg Terminal Data;   \\
 Morningstar Data   }\\
 \cmidrule{2-3}
& Personalized   Financial Advice & \parbox[t]{\linewidth}{
Financial Reports; \\
Investment Strategy Reports;  \\
Personal Financial Plans; \\
Risk Profile Reports; \\
Asset Performance Reports}  \\
% \cmidrule{2-3}
 & Risk management                 & \parbox[t]{\linewidth}{
 Financial Risk Analysis Reports; \\
 Basel III   Regulatory Filings; \\
 Value At Risk (VaR) Statements; \\
 Credit Default Swap (CDS)   Spreads; \\
 Stress Testing Reports }   \\
 \cmidrule{2-3}
& Regulatory   Compliance         & \parbox[t]{\linewidth}{
Legal Document Format; \\
Financial Report Format (FRF); \\
Risk Assessment Reports; \\
Regulatory Filings Format; \\
Compliance Audit  Reports   } \\ 
\midrule
\multirow{26}{*}{\shortstack[l]{Technology \\
and \\
Software}} & Web Design                      & \parbox[t]{\linewidth}{
HTML (HyperText Markup Language); \\
CSS (Cascading   Style Sheets); \\
JavaScript; \\
SVG (Scalable Vector Graphics); \\
.htaccess  }\\
\cmidrule{2-3}
 & Programming    & \parbox[t]{\linewidth}{
 Python Files (.py); \\
 JavaScript Files (.js); \\
 SQL   Files (.sql); \\
 Java Source Files (.java); \\
 C++ Source Code Files (.cpp)   } \\
 \cmidrule{2-3}
& UI/UX Design                    & \parbox[t]{\linewidth}{
UX/UI Mockup Annotation; \\
User Journey Mapping Text;   \\
Usability Test Session Transcripts; \\
UX/UI Design Specification (Typography   Palette etc.);\\
User Persona Description }  \\
\cmidrule{2-3}
 & Data Analysis                   & \parbox[t]{\linewidth}{
 SQL Result Set; \\
 Python Pandas DataFrame; \\
 R Data   Frame Output; \\
 Data Dictionary Output; \\
 Log File Output  } \\
 \cmidrule{2-3}
& Testing                         & \parbox[t]{\linewidth}{
Test Plan; \\
Test Case Description; \\
Bug/Issue Report;   \\
Test Summary Report; \\
Requirement Traceability Matrix (RTM)  }  \\ 
\midrule 
\multirow{10}{*}{\shortstack[l]{Commerce\\
and \\
Manufacturing}}          & E-commerce Personalization             & \parbox[t]{\linewidth}{
E-commerce Invoice Format; \\
Personalized Product Recommendation; \\
Shopping Cart Abandonment Reminder; \\
Shipping and Delivery Notification; \\
Customer Review and Rating Format  }\\
\cmidrule{2-3}
& Manufacturing Process Optimization     & \parbox[t]{\linewidth}{
Manufacturing Reports Format (MRF); \\
Bill of Materials (BOM); \\
Work Instruction Format (WIF); \\
Standard Operating Procedure (SOP); \\
Production Scheduling Format (PSF)   }       \\
% \cmidrule{2-3}
& Inventory and Supply Chain Management  & \parbox[t]{\linewidth}{
Purchase Order (PO) Format; \\
Inventory Report Format; \\
Sales Forecast Format; \\
Shipping Status Format; \\
Return/Replacement Order Format }   \\
\cmidrule{2-3}
& Quality Control                        & \parbox[t]{\linewidth}{
Product Inspection Report; \\
Quality Assurance (QA) Test Report; \\
Defect Tracking Log; \\
Product Compliance Certificate; \\
Supplier Quality Report  } \\
\cmidrule{2-3}
& Smart Logistics and Route Optimization & \parbox[t]{\linewidth}{
Freight Bill Format; \\
Inventory Update Format; \\
Shipping Manifest Format; \\
Route Optimization Report; \\
Order Pick List } \\ 
\midrule
\multirow{27}{*}{\shortstack[l]{Customer \\ Relationship \\ Management \\ (CRM)}} & Customer Service   & \parbox[t]{\linewidth}{
Customer Email Response Format; \\
Live Chat Transcript Format; \\
Customer Feedback Form Response Format;\\
Ticketing System Response Format; \\
Social Media Comment Response Format} \\
\cmidrule{2-3}
& Sales Forecasting                      & \parbox[t]{\linewidth}{
Sales Forecast Report; \\
Key Performance Indicator (KPI) Report; \\
Pipeline Report; \\
Sales Targets Report; \\
CRM Dashboard Summary }\\
\cmidrule{2-3}
& Recruitment Assistants                 &\parbox[t]{\linewidth}{
Resume Format; \\
Job Description Format; \\
Interview Schedule Format; \\
Applicant Status Update Format; \\
Candidate Comparative Analysis    }                                        \\
\cmidrule{2-3}
& Project Management                     & \parbox[t]{\linewidth}{
Gantt Chart Representation; \\
Task Breakdown Structure (TBS); \\
Project Status Reports; \\
Meeting Minutes; \\
Risk Assessment Reports       }                                         \\
\cmidrule{2-3}
 & Lead Scoring                           & \parbox[t]{\linewidth}{
 Lead Score Reports; \\
 Sales Funnel Analysis Documents; \\
 Lead Demographic Profiles; \\
 Customer Interaction Logs; \\
 Predictive Scoring Reports    }                                   \\ \midrule
\multirow{5}{*}{Marketing}                              & Consumer Behavior Analysis             & \parbox[t]{\linewidth}{
Consumer Behavior Report; \\
Marketing Performance Dashboard; \\
Advertising Copy Feedback; \\
Social Media Sentiment Analysis; \\
Competitor Analysis Summary    }                      \\
% \cmidrule{2-3}
& Advertising Campaign Optimization      & \parbox[t]{\linewidth}{
Advertising Audience Profile Format; \\
KPI Report Format;\\
A/B Test Result Format;\\
Competitive Analysis Format;\\
Campaign Budget Format    }  \\
\cmidrule{2-3}
& Content Curation and Creation          & \parbox[t]{\linewidth}{
Blog Post; \\
Social Media Post; \\
Email Newsletters; \\
Press Release; \\
SEO Content     }  \\
\cmidrule{2-3}
 & Social Media Management                & \parbox[t]{\linewidth}{
 Social Media Report; \\
 Content Calendar; \\
 User Sentiment Analysis; \\
 Hashtags Usage Report; \\
 Social Media Customer Inquiries Response }   \\
 \cmidrule{2-3}
& Search Engine Optimization (SEO)       & \parbox[t]{\linewidth}{
SERP (Search Engine Results Page) Report; \\
SEO Keyword Analysis; \\
On-Page SEO Audits; \\
Backlink Profile Report; \\
Competitor Analysis Report   }    \\ 
\midrule
\multirow{25}{*}{\shortstack[l]{Scientific \\
Research
and \\
Development}} & Mathematical Research                     & \parbox[t]{\linewidth}{
LaTeX;\\
MathML (Mathematical Markup Language);\\
SageMath Notebooks; \\
Maple; \\
MATLAB scripts    }\\
\cmidrule{2-3}
 & Physics   & \parbox[t]{\linewidth}{
 LaTeX (.tex); \\
 MathML (.mathml); \\
 BibTeX (.bib); \\
 Research Paper Abstract Structured Text; \\
 Physical Quantities and Units in UCUM (.ucum) }\\
 \cmidrule{2-3}
& Chemistry and Biological Sciences         & \parbox[t]{\linewidth}{
FASTA Format; \\
PDB Format (Protein Data Bank);\\
GenBank Format; \\
SMILES Format (Simplified Molecular Input Line Entry System); \\
MOL and SDF Formats (MOLecular and Structure-Data File)}        \\
\cmidrule{2-3}
 & Environmental Sciences and Climate Change & \parbox[t]{\linewidth}{
 Research Paper (APA Format); \\
 Scientific Report Format; \\
 Environmental Impact Statement (EIS); \\
 Peer Review Reports;\\
 Policy Briefs    }\\
 % \cmidrule{2-3}
 & Space Exploration                         & \parbox[t]{\linewidth}{
 NASA Planetary Data System (PDS) Format; \\
 MISSION OPERATION REPORT (MOR) Format; \\
 OBSErVation Time Series (OBSErVTS) Format; \\
 Spacecraft Event Language (SEL) Format; \\
 Telescope Observation Request (TOR) Format }              \\ 
 \midrule
\multirow{30}{*}{Education}                           & Adaptive Learning Platforms               & \parbox[t]{\linewidth}{
Personalized Learning Plan (PLP); \\
Assessment Results Format (ARF); \\
Interactive Course Content Format (ICCF);\\
Collaboration Log Format (CLF); \\
Task Progress Report Format (TPRF)  }                                           \\
\cmidrule{2-3}
  & Intelligent Tutoring Systems              & \parbox[t]{\linewidth}{
  Lesson Summary Format; \\
  Student Performance Report Format; \\
  Quiz/Instruction Format; \\
  Feedback/Correction Format; \\
  Personalized Learning Path Recommendation Format  } \\
  \cmidrule{2-3}
   & Automated Grading Systems                 & \parbox[t]{\linewidth}{
   Rubric Score Format; \\
   Student Report Format; \\
   Class Rank Format; \\
   Question Assessment Format; \\
   Error Analysis Format  } \\
   \cmidrule{2-3}
  & Education Data Analysis                   & \parbox[t]{\linewidth}{
  Report in Academic Results Format (ARF);\\
  Student Behavior Analysis Format (SBAF);\\
  Educational Content Analysis Format (ECAF);\\
  Learning Style Analysis Format (LSAF);\\
  Teaching Performance Evaluation Format (TPEF)   }       \\
  \cmidrule{2-3}
 & Language Learning                         & \parbox[t]{\linewidth}{
 Learning Material Format; \\
 Quizzes/Test Format; \\
 Progress Report Format; \\
 Language Translation Format; \\
 Phonetic Script Format     }   \\ 
 \midrule
\multirow{5}{*}{Legal}                               & Contract Review and Analysis              & \parbox[t]{\linewidth}{
Legal Brief Format; \\
Contract Abstract Format; \\
Risk Assessment Format; \\
Clause Breakdown Format; \\
Legal Opinion Format }\\
 \cmidrule{2-3}
 & Legal Document Automation                 & \parbox[t]{\linewidth}{
% Legal Document Format (.docx); \\
% Portable Document Format (.pdf);\\
 Legal XML (LegalXML); \\
% Rich Text Format (.rtf); \\
 Interactive Legal Applications Markup Language (iLAML)}                                                       \\
% \cmidrule{2-3}
& Legal Research                            & \parbox[t]{\linewidth}{
Legal Brief; \\
Case Citation; \\
Contract Format; \\
%Legal Memorandum; \\
Statute    }  \\
\cmidrule{2-3}
 & Predictive Legal Analytics                & \parbox[t]{\linewidth}{
 Legal Reporting Document; \\
 Case Brief Format; \\
 Legal Opinion Letter Format; \\
% Legal Memorandum Format; \\
 Legal Case Study Format          }                                                                                        \\
 \cmidrule{2-3}
 & Intellectual Property (IP) Management     & \parbox[t]{\linewidth}{
 Patent Disclosure Forms; \\
 Trademark Registration Documents; \\
 Copyright Registration Forms; \\
 Intellectual Property Agreement Contracts; \\
 Patent Litigation Documents       }   \\ 
 \midrule
\multirow{23}{*}{\shortstack[l]{Arts \\
and \\
Entertainment}}              & Music                                     & \parbox[t]{\linewidth}{
Lyrics Text Format; \\
Chord Sheet Format; \\
%Musical Score Text Format; \\
Tracklist Format; \\
Metadata Format }   \\
\cmidrule{2-3}
 & Film Scriptwriting                        & \parbox[t]{\linewidth}{
 Screenplay Format; \\
 Synopsis/Outline Format; \\
 Treatment Format; \\
 Beat Sheet Format; \\
 Character Profile/Backstory Format}   \\
 \cmidrule{2-3}
 & Visual Art Creation                       & \parbox[t]{\linewidth}{
 SVG (Scalable Vector Graphics); \\
 GLSL (OpenGL Shading Language);\\
 TikZ (code for creating vector graphics);\\
 POV-Ray Scene Description Language (SDL); \\
 G-code (a language in which people instruct computerized machine tools) }\\
 \cmidrule{2-3}
 & Video Game Development                    & \parbox[t]{\linewidth}{
 Game Design Document (GDD); \\
 Interactive Fiction Markup Language (IFML);\\
 Lua table for game configuration; \\
 GLSL Shader Code; \\
 Unreal Engine Blueprints Visual Scripting (Print String Node)    }                               \\
 % \cmidrule{2-3}
& Sports Analytics and Performance          & \parbox[t]{\linewidth}{
Game Statistics Report; \\
Training Performance Summary;\\
Player Ranking Report;\\
Injury Report; \\
Match Prediction Report        }     \\ %\midrule
\end{longtable}
\twocolumn
